Thermodynamic analysis and large-eddy simulations of LOx-CH4 and LOx-H2 flames at high pressure

Under rocket-relevant conditions, real-gas effects and thermodynamic non-idealities are prominent features of the flow field. Experimental investigations indicate that phase separation can occur depending on the operating conditions and on the involved species in the multicomponent flow. During the past decades, several research groups in the rocket combustion community have addressed this topic. In this contribution we employ a high-fidelity thermodynamic framework comprising real-gas and multicomponent phase separation effects to investigate liquid oxygen-methane and liquid oxygen-hydrogen flames at high pressure. A thorough introduction and discussion on multicomponent phase separation is conducted. The model is validated with experimental data and incorporated in a reacting flow CFD code. Thermodynamic effects are presented using one-dimensional counterflow diffusion flames. Both real-gas and phase separation effects are present and quantified in terms of derived properties. Finally, the method is applied in a three-dimensional large eddy simulation of a single-element reference test case and the results are compared to experimental data.

==> chapter_governingEquations.tex <==
%!TEX root = main.tex

\section{Governing Equations}


==> chapter_solver.tex <==
%!TEX root = main.tex

\section{Numerical Framework}

All simulations are performed with the open-source software package OpenFOAM that has been extended by the required combustion and thermodynamics models. The unstructured finite-volume code employs a PISO algorithm~\cite{Issa1991} to solve the governing equations. The mass conservation equation is not solved directly but used with the discretized momentum equation to derive a compressible pressure evolution equation guaranteeing mass conservation. This procedure reduces the stiffness of the system in the low Mach number region and allows for larger time steps. Variables are stored in the cell centers and Rhie-Chow interpolation is used to avoid checker-boarding of the pressure. A second-order accurate central differences scheme with the TVD-type van Leer limiter serves for spatial discretization. Temporal integration is performed using a second-order backward scheme. 




